Modeling Coordinated vs. P2P Mining: An Analysis of Inefficiency and Inequality in Proof-of-Work Blockchains

We study efficiency in a proof-of-work blockchain with non-zero latencies, focusing in particular on the (inequality in) individual miners' efficiencies. Prior work attributed differences in miners' efficiencies mostly to attacks, but we pursue a different question: Can inequality in miners' efficiencies be explained by delays, even when all miners are honest? Traditionally, such efficiency-related questions were tackled only at the level of the overall system, and in a peer-to-peer (P2P) setting where miners directly connect to one another. Despite it being common today for miners to pool compute capacities in a mining pool managed by a centralized coordinator, efficiency in such a coordinated setting has barely been studied. In this paper, we propose a simple model of a proof-of-work blockchain with latencies for both the P2P and the coordinated settings. We derive a closed-form expression for the efficiency in the coordinated setting with an arbitrary number of miners and arbitrary latencies, both for the overall system and for each individual miner. We leverage this result to show that inequalities arise from variability in the delays, but that if all miners are equidistant from the coordinator, they have equal efficiency irrespective of their compute capacities. We then prove that, under a natural consistency condition, the overall system efficiency in the P2P setting is higher than that in the coordinated setting. Finally, we perform a simulation-based study to demonstrate that even in the P2P setting delays between miners introduce inequalities, and that there is a more complex interplay between delays and compute capacities.

==> Makefile <==
MAIN=paper
SRCS=sections/*.tex

LMK=latexmk
OTYPE=-pdf
TEX=-pdflatex
TEX_OPTS="pdflatex -interaction=nonstopmode -shell-escape"
BIB=-bibtex

ERROR_MSG=Error: cannot find '$(LMK)' in path; try 'pdflatex $(MAIN).tex'

lmk_check =								\
	@which $(LMK) > /dev/null ||		\
		(echo "$(ERROR_MSG)" >& 2 &&	\
			exit 1)

default: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).tex $(SRCS)
	$(call lmk_check)
	@$(LMK) $(OTYPE) $(TEX)=$(TEX_OPTS) $(BIB) $<


# Automatically rebuild latex files whenever changes are made.
watch: $(MAIN).tex
	$(call lmk_check)
	@$(LMK) -pvc $(OTYPE) $(TEX)=$(TEX_OPTS) $(BIB) $<

clean:
	@rm -f *.dvi *.aux *.blg *.log *.ps *~ *.bbl *.fdb_latexmk *.fls $(MAIN).pdf *.out



BASE ?= orig
HEAD ?= HEAD

BASE_SHORT ?= $(shell git rev-parse --short ${BASE})
HEAD_SHORT ?= --

# (1) clone https://gitlab.com/git-latexdiff/git-latexdiff
# (2) cd git-latexdiff && make && make install
# (3) run 'make diff BASE=<version you want to compare against>'
diff:: 
	git latexdiff --main ${MAIN}.tex --latexmk  \
       ${BASE_SHORT} ${HEAD_SHORT} \
       -o ${MAIN}-diff.pdf \
       --ignore-latex-errors --view
#       --exclude-safecmd="todo,update"


.PHONY: watch clean


==> datastore/inefficiency/Makefile <==
R := Rscript

UTILS_DIR := ./utils
MEAS_DIR := ./meas
DATA_DIR := ./data
PLOTS_DIR := ./plots

# Base figures directory.
FIGS_DIR := ../../figures

# Output directory.
OUT_DIR := $(FIGS_DIR)/inefficiency


# Analyses.
ANALYSES := $(DATA_DIR)/two-nodes-stats.txt \
	$(DATA_DIR)/three-nodes-stats.txt       \
	$(DATA_DIR)/five-nodes-stats.txt

# Plots.
PLOTS := $(OUT_DIR)/two-nodes-stats.pdf \
	$(OUT_DIR)/three-nodes-stats.pdf    \
	$(OUT_DIR)/five-nodes-stats.pdf     \
	$(OUT_DIR)/cspeed-nodes-stats.pdf

ALL := $(ANALYSES) $(PLOTS)


.PHONY: all mostlyclean clean

all: $(ALL)

mostlyclean:
	rm -f $(PLOTS)

clean: mostlyclean
	rm -f $(ALL)


.DEFAULT_GOAL: all


# Compute basic stats on the efficiency of the system.
$(DATA_DIR)/%-nodes-stats.txt: $(UTILS_DIR)/eff-stats.R \
	$(MEAS_DIR)/%-nodes.csv
	@$(R) $^ $@


# Plot the stats on the efficiency of different configs.
$(OUT_DIR)/%-nodes-stats.pdf: $(PLOTS_DIR)/%-nodes-stats.gp \
	$(DATA_DIR)/%-nodes-stats.txt
	@gnuplot                        \
		-e 'IN_FILE="$(word 2, $^)' \
		-e 'OUT_FILE="$@'           \
		$(word 1, $^)


# Combine all measurements related to the cSpeed network into one file.
$(MEAS_DIR)/cspeed-nodes.csv: $(UTILS_DIR)/merge-eff-meas.R \
	$(MEAS_DIR)/five-nodes-ls.csv $(MEAS_DIR)/five-nodes-ls-600-20.csv
	@$(R) $^ $@


==> datastore/inequality/Makefile <==
R := Rscript

UTILS_DIR := ./utils
MEAS_DIR := ./meas
DATA_DIR := ./data
PLOTS_DIR := ./plots

# Lambdas for Bitcoin and Ethereum
BITCOIN_LAMBDA := 23684.2105
ETHEREUM_LAMBDA := 789.4737

# Base figures directory.
FIGS_DIR := ../../figures

# Output directory.
OUT_DIR := $(FIGS_DIR)/inequality


# Analyses.
ANALYSES := $(DATA_DIR)/two-nodes-stats.txt \
	$(DATA_DIR)/three-nodes-stats.txt       \
	$(DATA_DIR)/five-nodes-stats.txt

# Plots.
PLOTS := $(OUT_DIR)/two-nodes-stats.pdf  \
	$(OUT_DIR)/three-nodes-stats.pdf     \
	$(OUT_DIR)/five-nodes-stats.pdf      \
	$(OUT_DIR)/cspeed-nodes-stats.pdf    \
	$(OUT_DIR)/real-world-nodes-stats.pdf

ALL := $(ANALYSES) $(PLOTS)


.PHONY: all mostlyclean clean

all: $(ALL)

mostlyclean:
	rm -f $(PLOTS)

clean: mostlyclean
	rm -f $(ALL)


.DEFAULT_GOAL: all


# Compute basic stats on the inequality of the system.
$(DATA_DIR)/%-stats.txt: $(UTILS_DIR)/ineq-stats.R \
	$(MEAS_DIR)/%.csv
	@$(R) $^ $@


# Plot the stats on the inequality in the real-world scenario.
$(OUT_DIR)/real-world-nodes-stats.pdf: $(PLOTS_DIR)/real-world-nodes-stats.gp \
	$(DATA_DIR)/real-world-nodes-stats.txt
	@gnuplot                             \
		-e 'BITCOIN=$(BITCOIN_LAMBDA)'   \
		-e 'ETHEREUM=$(ETHEREUM_LAMBDA)' \
		-e 'IN_FILE="$(word 2, $^)'      \
		-e 'OUT_FILE="$@'                \
		$(word 1, $^)


# Plot the stats on the inequality in the real-world cSpeed scenario.
$(OUT_DIR)/cspeed-nodes-stats.pdf: $(PLOTS_DIR)/cspeed-nodes-stats.gp \
	$(DATA_DIR)/cspeed-nodes-stats.txt
	@gnuplot                             \
		-e 'BITCOIN=$(BITCOIN_LAMBDA)'   \
		-e 'ETHEREUM=$(ETHEREUM_LAMBDA)' \
		-e 'IN_FILE="$(word 2, $^)'      \
		-e 'OUT_FILE="$@'                \
		$(word 1, $^)


# Plot the stats on the inequality of different configs.
$(OUT_DIR)/%-stats.pdf: $(PLOTS_DIR)/%-stats.gp \
	$(DATA_DIR)/%-stats.txt
	@gnuplot                        \
		-e 'IN_FILE="$(word 2, $^)' \
		-e 'OUT_FILE="$@'           \
		$(word 1, $^)


# Combine all measurements related to the cSpeed network into one file.
$(MEAS_DIR)/cspeed-nodes.csv: $(UTILS_DIR)/merge-ineq-meas.R \
	$(MEAS_DIR)/five-nodes-ls.csv $(MEAS_DIR)/five-nodes-ls-600-20.csv
	@$(R) $^ $@

# Combine all measurements related to the real-world network into one file.
$(MEAS_DIR)/real-world-nodes.csv: $(UTILS_DIR)/merge-ineq-meas.R \
	$(MEAS_DIR)/five-nodes.csv $(MEAS_DIR)/five-nodes-ls-600-20.csv
	@$(R) $^ $@


==> datastore/real-world/Makefile <==
DATA_DIR := ./data
PLOTS_DIR := ./plots

# Base figures directory.
FIGS_DIR := ../../figures

# Output directory.
OUT_DIR := $(FIGS_DIR)/real-world


# Analyses.
ANALYSES :=

# Plots.
PLOTS := $(OUT_DIR)/real-world-nodes.pdf $(OUT_DIR)/real-world-nodes-no-observers.pdf

ALL := $(ANALYSES) $(PLOTS)


.PHONY: all mostlyclean clean

all: $(ALL)

mostlyclean:
	rm -f $(PLOTS)

clean: mostlyclean
	rm -f $(ALL)


.DEFAULT_GOAL: all


# Plot the locations of the real-world nodes on a map.
$(OUT_DIR)/real-world-nodes.pdf: $(PLOTS_DIR)/map.gp \
	$(DATA_DIR)/cities1.txt                           \
	$(DATA_DIR)/cities2.txt                           \
	$(DATA_DIR)/world-50m.txt
	@gnuplot                             \
		-e 'IN_FILE1="$(word 2, $^)'      \
		-e 'IN_FILE2="$(word 3, $^)'      \
		-e 'MAP_FILE="$(word 4, $^)'     \
		-e 'OUT_FILE="$@'                \
		$(word 1, $^)

# Plot the locations of the real-world nodes on a map.
$(OUT_DIR)/real-world-nodes-no-observers.pdf: $(PLOTS_DIR)/map-no-obs.gp \
	$(DATA_DIR)/cities1.txt                           \
	$(DATA_DIR)/world-50m.txt
	@gnuplot                             \
		-e 'IN_FILE1="$(word 2, $^)'      \
		-e 'MAP_FILE="$(word 3, $^)'     \
		-e 'OUT_FILE="$@'                \
		$(word 1, $^)


==> sections/app-100k.tex <==
\section{Length of the simulations}
\label{app.100k}
In our definition of the overall system efficiency \eqref{eq.efficiency.ind}, we define efficiency as $T \to \infty$. However our simulations naturally have finite length; we simulate the generation of $100,000$ blocks. In this appendix, we illustrate the speed of convergence of the efficiency as a function of $T$ to justify that our simulation length is sufficient to approximate $T\to\infty$. The results are shown for the P2P setting in Fig.~\ref{fig:p2p-simulation-length} and for the coordinated setting in  Fig.~\ref{fig:c-simulation-length} where the miners are equidistant from the coordinator. All plots show a cropped version of simulations up to $10,000$ blocks only. \PENDING{not really...}


\begin{figure*}[tb]
	\centering
	\begin{subfigure}[b]{\twocolgrid}
		\includegraphics[width={\textwidth}]{figures/simulation-length/p2p_h0.1_hash0.5-0.5.png}
		\figcap{}
	\end{subfigure}
	\begin{subfigure}[b]{\twocolgrid}
		\includegraphics[width={\textwidth}]{figures/simulation-length/p2p_h0.1_hash0.2-0.8.png}
		\figcap{}
	\end{subfigure}
	\begin{subfigure}[b]{\twocolgrid}
		\includegraphics[width={\textwidth}]{figures/simulation-length/p2p_h1_hash0.5-0.5.png}
		\figcap{}
	\end{subfigure}
	\begin{subfigure}[b]{\twocolgrid}
		\includegraphics[width={\textwidth}]{figures/simulation-length/p2p_h1_hash0.2-0.8.png}
		\figcap{}
	\end{subfigure}
    \begin{subfigure}[b]{\twocolgrid}
		\includegraphics[width={\textwidth}]{figures/simulation-length/p2p_h10_hash0.5-0.5.png}
		\figcap{}
	\end{subfigure}
	\begin{subfigure}[b]{\twocolgrid}
		\includegraphics[width={\textwidth}]{figures/simulation-length/p2p_h10_hash0.2-0.8.png}
		\figcap{}
	\end{subfigure}
	\figcap{(P2P setting) Efficiency as a function of simulation length in seconds for different $\lambda$s and hash power distributions}
	\label{fig:p2p-simulation-length}
\end{figure*}

\begin{figure*}[tb]
	\centering
	\begin{subfigure}[b]{\twocolgrid}
		\includegraphics[width={\textwidth}]{figures/simulation-length/c_h0.1_hash0.5-0.5.png}
		\figcap{}
	\end{subfigure}
	\begin{subfigure}[b]{\twocolgrid}
		\includegraphics[width={\textwidth}]{figures/simulation-length/c_h0.1_hash0.2-0.8.png}
		\figcap{}
	\end{subfigure}
	\begin{subfigure}[b]{\twocolgrid}
		\includegraphics[width={\textwidth}]{figures/simulation-length/c_h1_hash0.5-0.5.png}
		\figcap{}
	\end{subfigure}
	\begin{subfigure}[b]{\twocolgrid}
		\includegraphics[width={\textwidth}]{figures/simulation-length/c_h1_hash0.2-0.8.png}
		\figcap{}
	\end{subfigure}
    \begin{subfigure}[b]{\twocolgrid}
		\includegraphics[width={\textwidth}]{figures/simulation-length/c_h10_hash0.5-0.5.png}
		\figcap{}
	\end{subfigure}
	\begin{subfigure}[b]{\twocolgrid}
		\includegraphics[width={\textwidth}]{figures/simulation-length/c_h10_hash0.2-0.8.png}
		\figcap{}
	\end{subfigure}
	\figcap{(Coordinated setting) Efficiency as a function of simulation length in seconds for different $\lambda$s and hash power distributions, where the miners are equidistant from the coordinator.}
	\label{fig:c-simulation-length}
\end{figure*}

==> sections/app-coord.tex <==
\section{Coordinated Appendix} \label{s:coordinated_appendix}
\TODO{Polish the plots, unify the styles, drop the titles in Fig. 14}
\subsection{Coordinated communication model}
\TODO{Please write me ...}
\subsection{Coordinated mining}

So far, we focused on the P2P communications between miners and we have quantified the inequality and instability caused by network delays. We have shown that central miners (closer to the majority of nodes) have a non negligible advantages compared to the nodes farther away. Hitherto, communications within mining pools where abstracted out as we considered the net hashing power of a particular miner (or mining pool).

In this \TODO{appendix/section} we consider coordinated mining, where  miners will not be communicating with each other directly. Instead, all communications go through a coordinator. The Coordinator is responsible for assigning computational tasks to the miners and monitoring their proof of work. A variant of this model is used within mining pools as a way of coordinating mining nodes to collaborate on solving blocks for the P2P blockchain. (for more details, please refer to the stratum protocol \cite{stratum}).

\subsubsection{Overall System Efficiency}
\TODO{Clean-up the plots, have 1 legend only. -- Drop all $\lambda$s < 1?} 
We measure the overall pool efficiency in the coordinated setup as the total number of blocks $\hat{B_c}$ mined in time $t$ relative to the number of blocks $B$ that could have been mined at the same time $t$ had all coordinated nodes been at the coordinator's position $\eff_c \propto{} {|\hat{B_c}|}/{|B|}$.

To demonstrate the impact of network latencies on coordinated networks, we simulate a coordinated network of 2 miners and a coordinator. We vary the coordinator's position and measure the overall system efficiency for different $\lambda$s. We can see in Fig. \ref{fig:coordinated_global_efficiency} that the closer the coordinator to the majority of power the higher the overall coordinated system's efficiency becomes. \REMOVE{As a sanity check, we can also see that for very low $\lambda$s where the block generation rate is much higher than the block communication rate, that the efficiency of the systems drops close to zero.}

\subsubsection{Inequality in Efficiency}
As we have seen in the previous section, the overall coordinated system efficiency is highly affected by the coordinator's position. In this section, we would like to explore the how individual nodes' efficiency is affected. We measure a miner $i$'s efficiency in the coordinated setup as the total number of blocks $\hat{B_ci}$ mined in time $t$ relative to the number of blocks $B_i$ that could have been mined at the same time $t$ had all coordinated nodes been at the coordinator's position $\eff_ci \propto{} {|\hat{B_ci}|}/{|Bi|}$.

We guide this discussion by answering 2 questions: (1) How does the efficiency of a single node (and consequently, inequality) depend on the location of the coordinator? and (2) What is the location that results in the least inequality between nodes?

\parab{(1) How does the efficiency of a single node (and consequently, inequality) depend on the location of the coordinator?}

Let's focus on a single hardness to latency ratio, $\lambda = 1$, as we can see in Fig. \ref{fig:coordinated_equality}, the closer the coordinator to a node, the more efficient it becomes. Simply because it has a communication advantage. 

\parab{(2) What is the location that results in the least inequality between nodes?}

Since the communication ad/disadvantage is the root cause behind inequality, then we expect that an equidistant coordinator will result in complete equality, and this is indeed the case, as can be seen in Fig. \ref{fig:coordinated_equality}. This is the case as well with varying $\lambda$s and Hash power distributions.



==> sections/background.tex <==
\section{Background} \label{sec:background}

Bitcoin was introduced in 2008 by Satoshi
Nakamoto~\cite{Nakamoto-WhitePaper2008}, and it is the largest cryptocurrency in
the world in terms of market capitalization~\cite{CoinMarketCap-URL2019}.
A Bitcoin user or \newterm{client} issues transactions that move currency from
one or more addresses or \newterm{wallets} owned by the client to another
wallet.
Transactions issued by the clients are broadcast in a peer-to-peer network,
which connects the clients with the \newterm{miners}.
Miners validate the transactions and bundle them into a \newterm{block}, by
solving a cryptographic puzzle.
The solution to the crypto puzzle acts as the proof of miner's work---proof that
they invested significant computing power in mining the block.
A~block is a, typically non-empty, set of the broadcast transactions, and the
chain of blocks, with each pointing to an ancestor, constitutes the blockchain.

In return for ``mining'' a block and extending the blockchain miners get a block
reward. Users also voluntarily attach a fee with each transaction, to further
subsidize the miners, and miners reap this transaction fee upon inclusion (or
confirmation) of the concerned transaction.
Bitcoin is designed such that blocks are mined at a steady pace, $10$ minutes on
average, to keep the currency price stable~\cite{BitcoinWiki-Supply-URL2019}.
Mining rate is controlled by adjusting the \newterm{difficulty} of mining or
\newterm{hardness} of the cryptographic puzzle that miners have to solve to
create a block~\cite{BitcoinWiki-Diff-URL2017}.
The hardness (of the puzzle) is automatically adjusted, on average, every two
weeks (or every $\num{2016}$ blocks
mined)~\cite{BitcoinWiki-Diff-URL2017,BitcoinWisdom-WebArticle2019}.
In the rest of this paper, we use both hardness and difficulty to simply refer
to the average time spent in mining a block.

The chain of blocks is persisted across the miners in the network; there is no
central, trusted, storage facility for persisting the chain.
With a non-trivial probability, occasionally two or more miners may
simultaneously mine a block, causing a divergence in the chain. Such
disagreements on the contents of the chain also occur because of network
latencies: miners are connected to one another over a peer-to-peer network and
the messages announcing blocks across this network may reach different miners at
different times.
Miners resolve these conflicts by selecting, among all the options, the longest
chain; consequently, there may be brief periods of time where more than one
chain exists in the network, but eventually all miners will rally behind the
longest chain.
Mined blocks are, hence, not deemed \stress{confirmed} until they reach a
predefined \newterm{depth}, defined as the length of the chain (in terms of
blocks) from the tip (i.e., most recently added block) to the given block.
Once a block is confirmed, the transactions contained in the block are deemed
\stress{irrevocable}.
While the conventional wisdom in Bitcoin recommends a depth of $6$ blocks \cite{conventional-wisdom-6blocks} for considering a block irrevocable, there exists virtually no rationale or guidance on how to set this key parameter.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> sections/discussion.tex <==
\section{Concluding Remarks}\label{s:discussion}



==> sections/evaluation.tex <==
\section{Evaluation} \label{sec:eval}

\subsection{Simulator Design} \label{sec:simulator}
We build a blockchain Network Simulator (BCNS) that simulatessimulates the functions of a peer-to-peer blockchain network with respect to the mining interactions. BCNS is built as a discrete event loop. We assume an exponential distribution for the block generation time.
Simplifying assumptions:
\begin{itemize}
	\item No actual mining happens
	\item The probability of a miner mining a block is independent of the data in the block, and follows an exponential distribution.
	\item Block verification time is 0
	\item There are no transactions in the system
	\item Block propagation time is symmetric
	\item Propagation delay is based on the direct delay in the latency adjacency matrix, miners do not re-announce the arriving blocks
	\item All miners follow the protocol
	\item Miners receive blocks without asking for them
	\item Miners receive blocks without initial arrival of hashes
\end{itemize}


Simulator Inputs:
\begin{itemize}
	\item Distribution of computing capability -- AKA. hashing rate
	\item Hashing hardness -- AKA. mean block generation time
	\item Distribution of the compute capability -- Network latencies between nodes (Adjacency Matrix)
\end{itemize}
Simulator Outputs:
\begin{itemize}
	\item Global and per-node statistics:
	\begin{itemize}
		\item Total Number of blocks generated
		\item Total number of times a node had to switch chains
		\item Total number of orphaned blocks -> compute power wasted (wasted time * node compute capacity)
	\end{itemize}
	Efficiency (per node and global):
	\begin{itemize}
		\item Estimate 1: the total number of blocks in the longest chain/number of generated blocks
		\item Estimate 2: Total number of seconds wasted due to block orphaning + total number of seconds wasted due to mining a stale block
	\end{itemize}
	Convergence time:
	\begin{itemize}
		\item Convergence time of the system, the actual commit time.
	\end{itemize}
\end{itemize}

\subsection{Evaluation setting}
We evaluate the blockchain performance based on the following metrics

\begin{enumerate}[label=\alph*]
	\item Overall System Inefficiency -- measured as slow-down in the rate of growth of the longest chain vs optimal situation. Metric: Final chain length / Optimal chain length
	\item Inequality in how the inefficiency is distributed across computing elements -- measured as the slow-down in the rate of new blocks created per compute element. Per compute element efficiency is defined as the number of blocks included / number of blocks mined. We report the std deviation between compute elements
	\item Temporal instability from the perspective of different computing elements -- measured as the number of times the longest chain has been switched or the number of blocks in the  longest chains that were thought of as invalid over time (A measure of how frequently a soft fork happen as perceived by different miners). We report the rate of soft forking as: number of forks / final chain length
	\item Convergence time: When can we be certain that a block has been accepted by all nodes in the system. It is a measure of irrevocability in time. Measured as the time (max fork length * hardness) any observer has to wait before irrevocability can be guaranteed. We also show a distribution of probabilities of irrevocability as a heat map.
\end{enumerate}

Note: we collapse nodes that have 0 network delay into one node.


We start with a toy example to get the message across and then switch to larger simulations

%\subsection{Toy Example 1}
%
%Our toy example is based on just having 2 nodes of equal compute capacity
%
%\textit{\textbf{Overall System Inefficiency as hardness to latency change}}\\
%
%\begin{figure}[H]
%		\includegraphics[width={\linewidth}]{plots/toy_example_1_lambda_vs_efficiency}
%		\figcap{The effect of hardness to latency ratio on the overall efficiency of the system}
%		\label{fig:toy_1_lambda_eff}
%\end{figure}
%
%We can see in Fig. \ref{fig:toy_1_lambda_eff} that as the hardness to latency ($\lambda$) decrease, the less efficient the system becomes. For 2 nodes, the system can not be less efficient than 50\% because one of the 2 miners will eventually have a longer chain at the end of the simulation. 
%
%\textit{\textbf{Inequality in Inefficiency as hardness to latency change}}\\
%
%\begin{figure}[H]
%	\includegraphics[width={\linewidth}]{plots/toy_example_1_lambda_vs_miners_efficiency}
%	\figcap{The effect of hardness to latency ratio on the inequality of inefficiency of the system}
%	\label{fig:toy_1_lambda_eff_miners}
%\end{figure}
%We can see in Fig. \ref{fig:toy_1_lambda_eff_miners} that as the hardness to latency ($\lambda$) decrease, the inequality in miners efficiency is not affected because they are equally powerful.


\subsubsection{Demonstration Example with 2 miners}

\begin{figure}[H]
	\includegraphics[width={\linewidth}]{plots/2_miners_100K/infographic_nb}
	\figcap{A rough view of how the nodes are placed}
	\label{fig:toy_2_viz}
\end{figure}

Our toy example is based on just having 2 groups of nodes of varying compute capacities whith a setup similar to Fig \label{fig:toy_2_viz}.

The Fig. \label{fig:toy_2_viz} doesn't reflect the actual relative latency but is close to it.
Actual latencies:
\begin{itemize}
	\item M1-M2: 1 sec.
	\item OLM1 is 0.25 sec left of M1.
	\item ORM2 is 0.25 sec right of M2.
	\item OM1 is 0.25 sec right of M1, and 0.75 sec left of M2.
	\item OM is 0.5 sec right of M1, and 0.5 sec left of M2.
	\item OM2 is 0.75 sec right of M1, and 0.25 sec left of M2.
	\item OEQ is 1 sec away from both M1 and M2.
\end{itemize}

Nodes M1 and M2 are miners. Node M2 hashing power is always greater than or equal to M1's.



% \begin{figure}[H]
% 	\includegraphics[width={\linewidth}]{plots/2_miners_100K/overall_efficiency}
% 	\figcap{The effect of hardness to latency ratio on the overall efficiency of the system}
% 	\label{fig:toy_2_lambda_eff}
% \end{figure}
% We can see in Fig. \ref{fig:toy_2_lambda_eff} that as the hardness to latency ($\lambda$) increase, the more efficient the system becomes. For 2 nodes, the system can not be less efficient than 50\% because one of the 2 miners will eventually have a longer chain at the end of the simulation.
 

\textit{\textbf{Inequality in Inefficiency as hardness to latency change}}\\

% \begin{figure}[H]
% 	\includegraphics[width={\linewidth}]{plots/2_miners_100K/discrepancy_in_efficiency_std.png}
% 	\figcap{The effect of hardness to latency ratio on the inequality in inefficiency of the system}
% 	\label{fig:toy_2_lambda_eff_miners}
% \end{figure}
We can see in Fig. \ref{fig:toy_2_lambda_eff_miners} the std dev of miners efficiency. As the hardness to latency ($\lambda$) decrease, the inequality in miners efficiency becomes clear, especially for the configurations where miners have different compute capacity.


\textit{\textbf{Temporal instability as hardness to latency change for miners and observers}}

% \begin{figure*}
% 	\includegraphics[width={\linewidth}]{plots/2_miners_100K/temporal_instability_per_miner_fork_rate_vs_hpd_multi_line_plot}
% 	\figcap{The effect of hardness to latency ratio on the inequality in inefficiency of the system}
% 	\label{fig:toy_2_instability_vs_hpd}
% \end{figure*}

% \begin{figure*}
% 	\includegraphics[width={\textwidth}]{plots/2_miners_100K/temporal_instability_per_miner_fork_rate_multiplot}
% 	\figcap{The effect of hardness to latency ratio on the inequality in inefficiency of the system}
% 	\label{fig:toy_2_instability}
% \end{figure*}
% We can see in Fig. \ref{fig:toy_2_instability_vs_hpd} the per miner fork rate (defined as number of forks / chain length). Fig. \ref{fig:toy_2_instability}, however, shows the per miner fork rate for different ($\lambda$) configurations.

Usually observers have higher fork rates than actual miners. Observers are strongly impacted by nearer miners as well as more powerful miners. Stronger miners have more temporal stability than weaker miners. The number of forks is a function of an observer's latency to different miners (All observers that are equidistant from 2 miners will observe same number of forks)


\textit{\textbf{Convergence time as hardness to latency change}}\\


% \begin{figure*}
% 	\includegraphics[width={\linewidth}]{plots/2_miners_100K/convergence_time}
% 	\figcap{Convergence time for different miners}
% 	\label{fig:toy_2_convergence_time}
% \end{figure*}

% Fig. \ref{fig:toy_2_convergence_time} shows the convergence time computed as maximum number of orphans ever observed in a switch multiplied by the block mining time for that particular configuration.

\textit{\textbf{Quantifying the amount of time wasted mining while a new block was actually announced}}\\


% \begin{figure*}
% 	\includegraphics[width={\linewidth}]{plots/2_miners_100K/time_wasted_stale_delay_perc_multiplot}
% 	\figcap{Time wasted mining while a new block was actually announced}
% 	\label{fig:toy_2_time_wasted}
% \end{figure*}

% Fig. \ref{fig:toy_2_time_wasted} shows the amount of wasted time affecting each miner (trivial calculation would suffice here).

\subsubsection{Demonstration Example with 3 miners}

Our toy example is based on just having 3 equidistant groups of nodes of varying compute capacity, and an observing node at different positions as seen in Fig. \label{fig:toy_3_viz}.

\begin{figure}[H]
	\includegraphics[width={\linewidth}]{plots/3_miners_100K/infographic_nb}
	\figcap{A rough view of how the nodes are placed}
	\label{fig:toy_3_viz}
\end{figure}

The Fig. \label{fig:toy_3_viz} doesn't reflect the actual relative latency but is close to it.
Actual latencies:
\begin{itemize}
	\item M1-M2: 1 sec.
	\item OLM1 is 0.25 sec left of M1.
	\item ORM2 is 0.25 sec right of M2.
	\item OM1 is 0.25 sec right of M1, and 0.75 sec left of M2.
	\item OM is 0.5 sec right of M1, and 0.5 sec left of M2.
	\item OM2 is 0.75 sec right of M1, and 0.25 sec left of M2.
	\item M3 is 1 sec away from both M1 and M2.
\end{itemize}

Nodes M1, M2, and M3 are miners. M2 compute power is always >= M1 and M3's.



% \begin{figure}[H]
% 	\includegraphics[width={\linewidth}]{plots/3_miners_100K/overall_efficiency}
% 	\figcap{The effect of hardness to latency ratio on the overall efficiency of the system}
% 	\label{fig:toy_3_lambda_eff}
% \end{figure}

% We can see in Fig. \ref{fig:toy_3_lambda_eff} that as the hardness to latency ($\lambda$) increase, the more efficient the system becomes. For 2 nodes, the system can not be less efficient than 50\% because one of the 2 miners will eventually have a longer chain at the end of the simulation.


\textit{\textbf{Inequality in Inefficiency as hardness to latency change}}\\

% \begin{figure}[H]
% 	\includegraphics[width={\linewidth}]{plots/3_miners_100K/discrepancy_in_efficiency_std.png}
% 	\figcap{The effect of hardness to latency ratio on the inequality in inefficiency of the system}
% 	\label{fig:toy_3_lambda_eff_miners}
% \end{figure}
% We can see in Fig. \ref{fig:toy_3_lambda_eff_miners} the std dev of miners efficiency. As the hardness to latency ($\lambda$) decrease, the inequality in miners efficiency becomes clear, especially for the configurations where miners have different compute capacity.


\textit{\textbf{Temporal instability as hardness to latency change for miners and observers}}

\begin{figure*}
	\includegraphics[width={\linewidth}]{plots/3_miners_100K/temporal_instability_per_miner_fork_rate_vs_hpd_multi_line_plot}
	\figcap{The effect of hardness to latency ratio on the inequality in inefficiency of the system}
	\label{fig:toy_3_instability_vs_hpd}
\end{figure*}

\begin{figure*}
	\includegraphics[width={\textwidth}]{plots/3_miners_100K/temporal_instability_per_miner_fork_rate_multiplot}
	\figcap{The effect of hardness to latency ratio on the inequality in inefficiency of the system}
	\label{fig:toy_3_instability}
\end{figure*}
We can see in Fig. \ref{fig:toy_3_instability_vs_hpd} the per miner fork rate (defined as number of forks / chain length). Fig. \ref{fig:toy_3_instability}, however, shows the per miner fork rate for different ($\lambda$) configurations.

Usually observers have higher fork rates than actual miners. Observers are strongly impacted by nearer miners as well as more powerful miners. Stronger miners have more temporal stability than weaker miners. 

\textit{\textbf{Convergence time as hardness to latency change}}\\


\begin{figure*}
	\includegraphics[width={\linewidth}]{plots/3_miners_100K/convergence_time}
	\figcap{Convergence time for different miners}
	\label{fig:toy_3_convergence_time}
\end{figure*}

Fig. \ref{fig:toy_3_convergence_time} shows the convergence time computed as maximum number of orphans ever observed in a switch multiplied by the block mining time for that particular configuration.

% \textit{\textbf{Quantifying the amount of time wasted mining while a new block was actually announced}}\\


% \begin{figure*}
% 	\includegraphics[width={\linewidth}]{plots/3_miners_100K/time_wasted_stale_delay_perc_multiplot}
% 	\figcap{Time wasted mining while a new block was actually announced}
% 	\label{fig:toy_3_time_wasted}
% \end{figure*}

% Fig. \ref{fig:toy_3_time_wasted} shows the amount of wasted time affecting each miner (trivial calculation would suffice here).


\subsubsection{Demonstration Example with 3 non equidistant miners}

Our toy example is based on just having 3 groups of nodes of varying compute capacity, and an observing node at different positions, M3 is now 6 times farther away from M1, and M2 than M1 is From M2. Fig. \label{fig:toy_3f_viz}.

\begin{figure}[H]
	\includegraphics[width={\linewidth}]{plots/3f_miners_100K/infographic_nb}
	\figcap{A rough view of how the nodes are placed}
	\label{fig:toy_3f_viz}
\end{figure}

The Fig. \label{fig:toy_3f_viz} doesn't reflect the actual relative latency but is close to it.
Actual latencies:
\begin{itemize}
	\item M1-M2: 1 sec.
	\item OLM1 is 0.25 sec left of M1.
	\item ORM2 is 0.25 sec right of M2.
	\item OM1 is 0.25 sec right of M1, and 0.75 sec left of M2.
	\item OM is 0.5 sec right of M1, and 0.5 sec left of M2.
	\item OM2 is 0.75 sec right of M1, and 0.25 sec left of M2.
	\item M3 is 1 sec away from both M1 and M2.
\end{itemize}

Nodes M1, M2, and M3 are miners. M2 compute power is always >= M1 and M3's.



\begin{figure}[H]
	\includegraphics[width={\linewidth}]{plots/3f_miners_100K/overall_efficiency}
	\figcap{The effect of hardness to latency ratio on the overall efficiency of the system}
	\label{fig:toy_3f_lambda_eff}
\end{figure}

We can see in Fig. \ref{fig:toy_3f_lambda_eff} that as the hardness to latency ($\lambda$) increase, the more efficient the system becomes. For 2 nodes, the system can not be less efficient than 50\% because one of the 2 miners will eventually have a longer chain at the end of the simulation.


\textit{\textbf{Inequality in Inefficiency as hardness to latency change}}\\

\begin{figure}[H]
	\includegraphics[width={\linewidth}]{plots/3f_miners_100K/discrepancy_in_efficiency_std.png}
	\figcap{The effect of hardness to latency ratio on the inequality in inefficiency of the system}
	\label{fig:toy_3f_lambda_eff_miners}
\end{figure}
We can see in Fig. \ref{fig:toy_3f_lambda_eff_miners} the std dev of miners efficiency. As the hardness to latency ($\lambda$) decrease, the inequality in miners efficiency becomes clear, especially for the configurations where miners have different compute capacity.


\textit{\textbf{Temporal instability as hardness to latency change for miners and observers}}

\begin{figure*}
	\includegraphics[width={\textwidth}]{plots/3f_miners_100K/temporal_instability_heatmap_fork_rate}
	\figcap{The effect of hardness to latency ratio on the inequality in inefficiency of the system}
	\label{fig:toy_3f_instability}
\end{figure*}

 Fig. \ref{fig:toy_3f_instability}, however, shows the per miner fork rate for different ($\lambda$) configurations.

Usually observers have higher fork rates than actual miners. Observers are strongly impacted by nearer miners as well as more powerful miners. Stronger miners have more temporal stability than weaker miners. 

\textit{\textbf{Convergence time as hardness to latency change}}\\


\begin{figure*}
	\includegraphics[width={\linewidth}]{plots/3f_miners_100K/convergence_time}
	\figcap{Convergence time for different miners}
	\label{fig:toy_3f_convergence_time}
\end{figure*}

Fig. \ref{fig:toy_3f_convergence_time} shows the convergence time computed as maximum number of orphans ever observed in a switch multiplied by the block mining time for that particular configuration.

{\textbf{Quantifying the amount of time wasted mining while a new block was actually announced}}\\


\begin{figure*}
	\includegraphics[width={\linewidth}]{plots/3f_miners_100K/time_wasted_stale_delay_perc_multiplot}
	\figcap{Time wasted mining while a new block was actually announced}
	\label{fig:toy_3f_time_wasted}
\end{figure*}

Fig. \ref{fig:toy_3f_time_wasted} shows the amount of wasted time affecting each miner (trivial calculation would suffice here).


\subsubsection{Real life simulations}

Bitcoin operates at a hardness to latency range ($\lambda$) of 100 to 1000, while Ethereum for instance operates at the range 10 to 100.
Based on the top 19 Mining pools as reported by btc.com on May 23rd for a month period of time \footnote{https://btc.com/stats/pool?pool\_mode=month}. 

Assuming an exponential network delays with a mean of 300ms, we have the following results:

\begin{figure}[H]
	\includegraphics[width={\linewidth}]{plots/real_exp_latD_100K/infographic_nb}
	\figcap{A rough view of how the nodes are placed}
	\label{fig:real_exp_viz}
\end{figure}

The Fig. \label{fig:real_exp_viz} doesn't reflect the actual relative latency but is close to it.



\begin{figure}[H]
	\includegraphics[width={\linewidth}]{plots/real_exp_latD_100K/overall_efficiency}
	\figcap{The effect of hardness to latency ratio on the overall efficiency of the system}
	\label{fig:real_exp_lambda_eff}
\end{figure}

We can see in Fig. \ref{fig:real_exp_lambda_eff} that as the hardness to latency ($\lambda$) increase, the more efficient the system becomes. For 2 nodes, the system can not be less efficient than 50\% because one of the 2 miners will eventually have a longer chain at the end of the simulation.


\textit{\textbf{Inequality in Inefficiency as hardness to latency change}}\\

\begin{figure}[H]
	\includegraphics[width={\linewidth}]{plots/real_exp_latD_100K/discrepancy_in_efficiency_std.png}
	\figcap{The effect of hardness to latency ratio on the inequality in inefficiency of the system}
	\label{fig:real_exp_lambda_eff_miners}
\end{figure}
We can see in Fig. \ref{fig:real_exp_lambda_eff_miners} the std dev of miners efficiency. As the hardness to latency ($\lambda$) decrease, the inequality in miners efficiency becomes clear, especially for the configurations where miners have different compute capacity.


\textit{\textbf{Temporal instability as hardness to latency change for miners and observers}}


\begin{figure*}
	\includegraphics[width={\textwidth}]{plots/real_exp_latD_100K/temporal_instability_heatmap_fork_rate}
	\figcap{The effect of hardness to latency ratio on the inequality in inefficiency of the system}
	\label{fig:real_exp_instability}
\end{figure*}
 Fig. \ref{fig:real_exp_instability}, however, shows the per miner fork rate for different ($\lambda$) configurations.

Usually observers have higher fork rates than actual miners. Observers are strongly impacted by nearer miners as well as more powerful miners. Stronger miners have more temporal stability than weaker miners. 

\textit{\textbf{Convergence time as hardness to latency change}}\\


\begin{figure*}
	\includegraphics[width={\linewidth}]{plots/real_exp_latD_100K/convergence_time}
	\figcap{Convergence time for different miners}
	\label{fig:real_exp_convergence_time}
\end{figure*}

Fig. \ref{fig:real_exp_convergence_time} shows the convergence time computed as maximum number of orphans ever observed in a switch multiplied by the block mining time for that particular configuration.

\textit{\textbf{Quantifying the amount of time wasted mining while a new block was actually announced}}\\


\begin{figure*}
	\includegraphics[width={\linewidth}]{plots/real_exp_latD_100K/time_wasted_stale_delay_perc_multiplot}
	\figcap{Time wasted mining while a new block was actually announced}
	\label{fig:real_exp_time_wasted}
\end{figure*}

Fig. \ref{fig:real_exp_time_wasted} shows the amount of wasted time affecting each miner (trivial calculation would suffice here).


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> sections/instability.tex <==
\begin{figure*}[tb]
	\centering
	\begin{subfigure}[b]{\twocolgrid}
		\includegraphics[width={0.8\textwidth}]{{figures/illustrations/two-nodes.pdf}}
		\sfigcap{Two-node P2P scenario with observers}
		\label{fig:two-node-obs}
	\end{subfigure}
  \begin{subfigure}[b]{\twocolgrid}
    \includegraphics[trim={90 90 60 20}, width={\textwidth}, height={3.5cm}, clip]{{figures/real-world/real-world-nodes.pdf}}  
    \vspace{.2cm}
    \sfigcap{}
    \label{fig:real-world-obs}
  \end{subfigure}
	\figcap{Topology of the network (not drawn to scale) showing the miners (in red) and observers (in blue) as well as the network delays between them in the two-node and a real-world scenarios.}
\end{figure*}

\begin{figure*}[tb]
	\centering
	\begin{subfigure}[b]{\twocolgrid}
		\includegraphics[width={\textwidth}]{{figures/instability/instability-two-node-num-forks-gini_02}}
		\figcap{}
		\label{fig:two-node-inst-02}
	\end{subfigure}
	\begin{subfigure}[b]{\twocolgrid}
		\includegraphics[width={\textwidth}]{{figures/instability/instability-two-node-num-forks-gini_04}}
		\figcap{}
		\label{fig:two-node-inst-04}
	\end{subfigure}
	\begin{subfigure}[b]{\twocolgrid}
		\includegraphics[width={\textwidth}]{{figures/instability/instability-two-node-max-forks-gini_02}}
		\figcap{}
		\label{fig:two-node-inst-02-depth}
	\end{subfigure}
	\begin{subfigure}[b]{\twocolgrid}
	\includegraphics[width={\textwidth}]{{figures/instability/instability-two-node-max-forks-gini_04}}
	\figcap{}
	\label{fig:two-node-inst-04-depth}
	\end{subfigure}
%	\begin{subfigure}[b]{\twocolgrid}
%		\includegraphics[width={\textwidth}]{figures/instability-fc/instability-five-node-num-forks-gini_05.pdf}
%		\figcap{}
%		\label{fig:multi-node-inst}
%	\end{subfigure}
%	\begin{subfigure}[b]{\twocolgrid}
%		\includegraphics[width={\textwidth}]{figures/instability-fc/instability-five-node-num-forks-gini_06.pdf}
%		\figcap{}
%		\label{fig:multi-node-inst_06}
%	\end{subfigure}
	\figcap{(P2P) Effect of hardness-to-latency ratio $(\lambda)$ and the relative position of an observer on the perceived stability of the system for ($\gamma_h=0.2$) in (a,c) , and for ($\gamma_h=0.4$) in (b,d) }
\end{figure*}

%\begin{figure*}[tb]
%	\center
%	\begin{subfigure}[b]{\twocolgrid}
%		\includegraphics[width={\textwidth}]{figures/instability-fc/instability-two-node-max-forks-gini_02.pdf}
%		\figcap{}
%		\label{fig:two-node-inst-02-max}
%	\end{subfigure}
%	\begin{subfigure}[b]{\twocolgrid}
%		\includegraphics[width={\textwidth}]{figures/instability-fc/instability-two-node-max-forks-gini_04.pdf}
%		\figcap{}
%		\label{fig:two-node-inst-04-max}
%	\end{subfigure}
%	\begin{subfigure}[b]{\twocolgrid}
%		\includegraphics[width={\textwidth}]{figures/instability-fc/instability-five-node-max-forks-gini_05.pdf}
%		\figcap{}
%		\label{fig:multi-node-inst-max}
%	\end{subfigure}
%	\begin{subfigure}[b]{\twocolgrid}
%		\includegraphics[width={\textwidth}]{figures/instability-fc/instability-five-node-max-forks-gini_06.pdf}
%		\figcap{}
%		\label{fig:multi-node-inst_06-max}
%	\end{subfigure}
%	\figcap{Effect of hardness-to-latency ratio $(\lambda)$ and the relative position
%		of an observer on the measure of stability (Maximum fork depth) in (a) two-node ($G=0.2$), (b)
%		two-node ($G=0.4$), (c) real-world ($G=0.5$), and (d)  (c) real-world ($G=0.62$) scenarios. }
%\end{figure*}

\section{Instability}\label{s:instability}


\begin{figure*}[tb]
	\centering
	\begin{subfigure}[b]{\threecolgrid}
		\includegraphics[width={\textwidth}]{{figures/instability/five-nodes-stats_g0.62_number_of_forks_cdf.pdf}}
		\figcap{}
		\label{fig:15_miners_num_of_forks_cdf_g62}
	\end{subfigure}
	\begin{subfigure}[b]{\threecolgrid}
		\includegraphics[width={\textwidth}]{{figures/instability/five-nodes-stats_g0.00_number_of_forks_cdf.pdf}}
		\figcap{}
		\label{fig:15_miners_num_of_forks_cdf_g00}
	\end{subfigure}
	\begin{subfigure}[b]{\threecolgrid}
		\includegraphics[width={\textwidth}]{{figures/instability/five-nodes-stats_g0.62max_depth_of_forks_cdf.pdf}}
		\figcap{}
		\label{fig:15_miners_depth_of_forks_cdf_g62}
	\end{subfigure}

	\figcap{(P2P) CDFs showing the instability measures for (a) number of forks ($\gamma_h=0.62$), (b)number of forks ($\gamma_h=0$), and (c) Maximum observed fork depth ($\gamma_h=0.62$) across different nodes for different $\lambda$s in the Real-World scenario.}
	\label{fig:instability_15_240_g062}
\end{figure*}
\begin{figure*}[tb]
	\centering
	\begin{subfigure}[b]{\threecolgrid}
		\includegraphics[width={\textwidth}]{{figures/instability/five-nodes-stats_g0.00max_depth_of_forks_cdf.pdf}}
		\figcap{}
		\label{fig:15_miners_depth_of_forks_cdf_g00}
	\end{subfigure}
	\begin{subfigure}[b]{\threecolgrid}
		\includegraphics[width={\textwidth}]{{figures/instability/world-capitals_g0.00_number_of_forks_cdf.pdf}}
		\figcap{}
		\label{fig:world_capitals_num_of_forks_cdf}
	\end{subfigure}
	\begin{subfigure}[b]{\threecolgrid}
		\includegraphics[width={\textwidth}]{{figures/instability/world-capitals_g0.00max_depth_of_forks_cdf.pdf}}
		\figcap{}
		\label{fig:world_capitals_depth_of_forks_cdf}
	\end{subfigure}
	\figcap{(P2P) CDFs showing the instability measures for (a) Maximum observed fork depth ($\gamma_h=0$) in the Real-World scenario ($\gamma_h=0$). (b, c) Number of forks and maximum fork depth when considering equally powerful miners in the 240 World country capitals ($\gamma_h=0$)}
	\label{fig:instability_15_240_g0}
\end{figure*}
In the context of P2P mining, the network delays between miners fundamentally alters measures of stability.
%
Blockchains guarantee irrevocable transactions---a key reason for their widespread adoption.
%
Forks in the chain are, however, inevitable, and they impact the irrevocability of transactions:
Since miners eventually fall behind the longest chain, transactions in shorter chains following the fork, despite being committed in blocks, are essentially
revoked unless they are also included in some other block in the longest chain.
%
Unsurprisingly, transactions are not deemed \stress{confirmed}, until much
later---until the block $b_i$ in which they are committed is adjoined by $n$
other blocks in the chain.
%
The constant $n$ defines the \term{depth} of the block $b_i$ as well as the
transactions contained in that block.
%
The rationale behind the choice of $n$ is that the likelihood of a fork affecting a transaction that is $n$-blocks deep is infeasible, if not impossible, for any user in the network.
%
Conventional wisdom in Bitcoin, for instance, uses a system-wide depth of $6$ blocks for confirmation.
%
We show, nevertheless, that this system-wide assumption does not hold water.

\begin{figure*}[tpb]
    \centering
    \includegraphics[width=2.8in]{{illustrations/two-nodes-with-obs}}
    \figcap{(P2P) Although the observer (blue square) views $m_2$ extending the chain,
      $m_1$'s longer sequence of blocks eventually end up replacing $m_2$'s
      block. The observer witnesses many such changes (or forks) in the chain
      over time (much more than when she is in close proximity to $m_1$) and may
      conclude that the chain is unstable (i.e., blocks are highly likely to be
      replaced).}
    \label{fig:two-nodes-with-obs-instability}
\end{figure*}

We demonstrate, using the notion of a neutral observer (i.e., a user or
participant who does not participate in mining blocks), that the choice of a
single system-wide constant is irrational.
%
Let us consider the illustration (Fig.~\ref{fig:two-nodes-with-obs-instability})
and suppose that a neutral observer (in blue) is situtated between the two
miners: $m_1$ and $m_2$.
%
If the observer is in close proximity to $m_1$, i.e., $d_1 \ll d_2$, the
observer will see, except on rare occasions, the blockchain being extended only
by $m_1$.
%
If, however, she is close to $m_2$, i.e., $d_1 \gg d_2$, the observer might see
a block from $m_2$ every now and then.
%
She, nevertheless, will also witness $m_2$'s blocks replaced in the chain by
$m_1$'s (longer) sequence of blocks.
%
The number as well as depth of forks witnessed by the observer significantly
varies as a function of his or her relative position with respect to the miners
in the network.
%
The need for an instability measure that accounts for the relative position of
an observer fundamentally changes the design and operation of the blockchains.


Each miner, or more generally, each observer has a local ``view'' of the
blockchain based on the announcements of blocks that she receives.
Observers in a blockchain (e.g., Bitcoin and Ethereum) arrive at a consensus by
falling behind the longest chain.
Whenever an observer receives an announcement of a longer chain, she switches to
this new longer chain.
Generally, newly mined blocks lengthen the chain by one block, but such
extensions do not throw away any work on the older chain.
% Due to the inherent randomization in the ``mining'' process and factors such as
% network delays, 
Every now and then, two or more miners may, however, announce a new block at roughly the
same time and introduce forks (i.e., extend the chain with multiple tails).
While forks are eventually resolved, when one of the tail ends up being longer
than the other, the work done (i.e., blocks in the other tails) is thrown out.

The number of forks witnessed by an observer measures the instability of the
system, since each fork results in \stress{orphaning} a non-zero number of
blocks.
We distributed observers uniformly on the two-dimensional plane
containing the two-node topology \ref{fig:two-node-obs}.
Figs.~\ref{fig:two-node-inst-02}~\&~\ref{fig:two-node-inst-04} show the maximum
number of forks observed at three different locations; $RM1$ and $LM_{2}$ were close
to either nodes, while $CM_{12}$ was midway between the nodes. It suffices to shows
only a subset since our intent is to only confirm the variations in observations
depending on location.
The figures depict different hashing-power distributions across the nodes; with
Fig.~\ref{fig:two-node-inst-02} associated with Gini coefficient $G{=}0.2$ and
Fig.~\ref{fig:two-node-inst-04} to $G{=}0.4$.
The observers observe significantly different number of forks, and if hashing
power is uniformly distributed $CM_{12}$ observes more forks than either $RM_{1}$ or
$LM_{2}$. \REVIEW{$EM_{12}$ observes the same instability as that of $CM_{12}$ because it is equidistant from both miners, and as such will be having the same, but delayed, view of $CM_{12}$.} 

The discrepancy in the observers perspectives becomes more worrisome in the
real-world scenario \ref{fig:real-world-obs} in Fig.~\ref{fig:instability_15_240_g062},~\ref{fig:instability_15_240_g0}.
Interestingly, at higher values of $\lambda$, where Bitcoin and Ethereum operate, the
variance across the observers still exists.
Our inferences also hold true for the observers' measure of 
number of forks as well as the maximum number of orphaned blocks observed in a fork.
The significant variance in observations of instability calls to question the
widespread conventional wisdom of choosing $6$ blocks in Bitcoin as sufficient (or required)
depth for deeming blocks as confirmed. In fact, the number of blocks a transaction requires to 
be considered confirmed should take into consideration the sender and receiver geographic location and connectivity to the rest of the network.

In Practice, Bitcoin observed a max 4 blocks deep fork (except for a bug that caused a 53 block deep chain to be orphaned). In Our simulations also show that for a hardness of 100-1000, in over 1 Million blocks, no more than 3 block was ever orphaned. See Fig. ~\ref{fig:instability_15_240_g062},~\ref{fig:instability_15_240_g0}.

\paraib{Implications}
Instability is a metric that impacts both miners and observers adversely. A stable system would allow miners to always work on the latest announced block without risking there work getting discarded (in case of competing blocks). Similarly, Observers, or clients can consider a transaction confirmed without unnecessarily waiting for longer durations of time. The fact that the system's instability is a function of where the observer is located complicates the trust users might be willing to put in the system.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


%
%\begin{figure*}[tb]
%	\center
%	\begin{subfigure}[b]{\twocolgrid}
%		\includegraphics[width={\textwidth}]{figures/instability/instability_CDFs/15_miners_btc_number_of_forks_cdf.pdf}
%		\figcap{}
%		\label{fig:15_miners_btc_number_of_forks_cdf}
%	\end{subfigure}
%	\begin{subfigure}[b]{\twocolgrid}
%		\includegraphics[width={\textwidth}]{figures/instability/instability_CDFs/15_miners_ls_btc_number_of_forks_cdf.pdf}
%		\figcap{}
%		\label{fig:15_miners_ls_btc_number_of_forks_cdf}
%	\end{subfigure}
%	\begin{subfigure}[b]{\twocolgrid}
%		\includegraphics[width={\textwidth}]{figures/instability/instability_CDFs/100_cities_btc_number_of_forks_cdf.pdf}
%		\figcap{}
%		\label{fig:100_cities_btc_number_of_forks_cdf}
%	\end{subfigure}
%	\begin{subfigure}[b]{\twocolgrid}
%		\includegraphics[width={\textwidth}]{figures/instability/instability_CDFs/world_capitals_btc_number_of_forks_cdf.pdf}
%		\figcap{}
%		\label{fig:world_capitals_btc_number_of_forks_cdf}
%	\end{subfigure}
%	\figcap{CDF of number of forks observed by different nodes in Bitcoin like setting for (a) Real-World scenario ($G=0.62$) (b) Real-World scenario with non inflated speed of light latencies ($G=0.62$), (c) 100 random cities \cite{simplemaps_100cities} ($G=0$), and (d) 240 World country capitals ($G=0$).}
%	\label{fig:btc_number_of_forks_cdf}
%\end{figure*}
%
%\begin{figure*}[tb]
%	\center
%	\begin{subfigure}[b]{\twocolgrid}
%		\includegraphics[width={\textwidth}]{figures/instability/instability_CDFs/15_miners_eth_number_of_forks_cdf.pdf}
%		\figcap{}
%		\label{fig:15_miners_eth_number_of_forks_cdf}
%	\end{subfigure}
%	\begin{subfigure}[b]{\twocolgrid}
%		\includegraphics[width={\textwidth}]{figures/instability/instability_CDFs/15_miners_ls_eth_number_of_forks_cdf.pdf}
%		\figcap{}
%		\label{fig:15_miners_ls_eth_number_of_forks_cdf}
%	\end{subfigure}
%	\begin{subfigure}[b]{\twocolgrid}
%		\includegraphics[width={\textwidth}]{figures/instability/instability_CDFs/100_cities_eth_number_of_forks_cdf.pdf}
%		\figcap{}
%		\label{fig:100_cities_eth_number_of_forks_cdf}
%	\end{subfigure}
%	\begin{subfigure}[b]{\twocolgrid}
%		\includegraphics[width={\textwidth}]{figures/instability/instability_CDFs/world_capitals_eth_number_of_forks_cdf.pdf}
%		\figcap{}
%		\label{fig:world_capitals_eth_number_of_forks_cdf}
%	\end{subfigure}
%	\figcap{CDF of number of forks observed by different nodes in Ethereum like setting for (a) Real-World scenario ($G=0.62$) (b) Real-World scenario with non inflated speed of light latencies ($G=0.62$), (c) 100 random cities \cite{simplemaps_100cities} ($G=0$), and (d) 240 World country capitals ($G=0$).}
%	\label{fig:eth_number_of_forks_cdf}
%\end{figure*}


==> sections/methodology.tex <==
\section{Methodology} \label{sec:methodology}

We evaluate the blockchains performance based on the following metrics:
\begin{enumerate}[label=\alph*]
	\item Overall System Inefficiency -- measured as slow-down in the rate of growth of the longest chain vs optimal situation
	\item Inequality in how the inefficiency is distributed across computing elements -- measured as the slow-down in the rate of new blocks created per compute element
	\item Temporal instability from the perspective of different computing elements -- measured as the number of times the longest chain has been switched or the number of blocks in the  longest chains that were thought of as invalid over time
	\item Convergence time: When can we be certain that a block has been accepted by all nodes in the system
\end{enumerate}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> sections/misc.tex <==
--- FORMER TEXT WITH TWO DEFINITIONS---\\
We consider two alternative definitions of the efficiency of miner $i$:
\begin{equation*}
e_i^1 = \frac{\hat{B}_i}{B_i}, \quad \textrm{ and } \quad e_i^2 = \frac{\hat{B}_i}{h_iT/\tau}.
\end{equation*}
In both definitions, the efficiency is a random variables where the numerator is the number of blocks mined under the mining model used that are useful, i.e., that are included in the longest chain. In the second definition, the denominator $h_iT/\tau$ represents the average number of blocks that the miner would have mined within the time window of length $T$ if it was alone, while in the first the denominator is $B_i$, the actual number of blocks mined under the mining model used. Note that due to the memoryless property of the exponential distribution, $B_i$ converges almost surely towards $h_iT/\tau$ as $T$ goes to infinity, hence both definitions are equivalent in the P2P mining model where the miners never stop mining. \TODO{Move to The discussion in \ref{s:inequality} to explain how we measure the inefficiency in Ethereum}

\bigskip 
\bigskip
\bigskip

OLD TEXT BELOW

Notwithstanding the numerous applications of blockchain, concerns of the
system's energy consumption is rife in scientific literature and discussions.
%
The \underline{C}ambridge \underline{B}itcoin \underline{E}lectricity
\underline{C}onsumption \underline{I}ndex (CBECI) estimates, for instance, the
energy consumption of Bitcoin to be higher than that of many other countries,
e.g., Finland, Belgium, and Switzerland~\cite{CBECI-WebArticle2019}.
%
Prior work characterized the efficiency (or the lack thereof) of the system, by
comparing the energy spent to confirm a set of transactions between two entities
to that of a conventional banking system.
%
The global or system-level measure of inefficiency in these studies, estimated
based on the blocks added to the chain misses a crucial point—the failed
attempts of individual miners to add a block to the chain.
%
Such failed attempts are typically not recorded on the chain, and hence not
accounted for in prior studies.
%
Virtually all prior work ignore the subtle, but non-trivial, effect of network
delays (or latencies) on the inefficiency of an individual miner.


Latencies experienced by miners (or mining pools) to exchange data with other
miners are not the same or even similar.
%
It stands to reason then to question the implications of the latencies
experienced by a miner on his/her inefficiency.
% %
% Since pairwise latencies between miners are not uniform, inefficiency is not distributed uniformly across the miners.
% %
% Most important, inefficiency is not a function of strictly a miner's hashing
% power.
% %
We show, through illustrations and simulations, that the relative position of a
miner in the network, imputed by the latency matrix comprising pairwise
latencies between all miners, affects the miners inefficiency.
%
Simply by virtue of his or her position a miner may be more (or less) efficient
than expected from their hashing power.
% %
% Most important, the miners' relative positions in the network introduces
% unfairness in inefficiency across the system.
% %
We capture the inequality (in inefficiency) in \(\gamma{} \in{} [0, 1]\), where
\(\gamma{} = 0\) implies a uniform and \(\gamma{} = 1\) indicates a highly
skewed distribution of inefficiencies.
%
Suppose that the blocks mined by a miner $m_i$ with hashing power $h_i$ during a
time period $t$ is $B_i$.
%
The subset $\hat{B_i}$ of $B_i$ that are added to the longest chain estimates
the efficiency of the miner, $e_{i} \propto{} {|\hat{B_i}|}/{|B_i|}$.
%
Then, we derive the distribution of inefficiency $\eta_i = 1-\eff_i$ across all
miners using the Gini coefficient~\cite{Wiki-WebArticle2019}.

While the global inefficiency of blockchains is well-known, the inherent
unfairness in inefficiency of miners, introduced by their relative positions in
the network, has never been studied before.
%
Let us consider a hypothetical blockchain network with only two miners, $m_1$
and $m_2$ as seen in Fig.~\ref{fig:two-nodes-with-obs-instability}.
%
Suppose that the hashing power of $m_1$ is much larger than that of $m_2$.
%
If we also suppose that the blocks generated by each miner is advertised to the other instantaneously (i.e., with \stress{zero} delay), each miner will, in expectation, proportional to their hashing power.
%
High network delays between the miners, in contrast, will deprive $m_2$ of
virtually all opportunities to mine a block:
By the time $m_2$'s announcement of a new block reaches $m_1$, the latter may
have generated one or more blocks, disposing all of $m_2$'s efforts.
%
This inequality in inefficiency imparted by the network delays has far reaching
implications for deployment as well as security of the mining infrastructure.


Besides introducing inequality in inefficiency, the network delays between
miners fundamentally alters measures of stability.
%
Blockchains guarantee irrevocable transactions---a key reason for their
widespread adoption.
%
Forks in the chain are, however, inevitable, and they impact the irrevocability
of transactions:
Since miners eventually fall behind the longest chain, transactions in shorter
chains following the fork, despite being committed in blocks, are essentially
revoked unless they are also included in some other block in the longest chain.
%
Unsurprisingly, transactions are not deemed \stress{confirmed}, until much
later---until the block $b_i$ in which they are committed is adjoined by $n$
other blocks in the chain.
%
The constant $n$ defines the \term{depth} of the block $b_i$ as well as the
transactions contained in that block.
%
The rationale behind the choice of $n$ is that the likelihood of a fork
affecting a transaction that is $n$-blocks deep is infeasible, if not
impossible, for any user in the network.
%
Conventional wisdom in Bitcoin, for instance, uses a system-wide depth of $6$
blocks for confirmation.
%
We show, nevertheless, that this system-wide assumption does not hold water.


We demonstrate, using the notion of a neutral observer (i.e., a user or
participant who does not participate in mining blocks), that the choice of a
single system-wide constant is irrational.
%
Let us revert to the earlier illustration (Fig.~\ref{fig:two-nodes-with-obs-instability})
and suppose that a neutral observer (in blue) is situtated between the two
miners.
%
If the observer is in close proximity to $m_1$, i.e., $d_1 \ll d_2$, the
observer will see, except on rare occasions, the blockchain being extended only
by $m_1$.
%
If, however, she is close to $m_2$, i.e., $d_1 \gg d_2$, the observer might see
a block from $m_2$ every now and then.
%
She, nevertheless, will also witness $m_2$'s blocks replaced in the chain by
$m_1$'s (longer) sequence of blocks.
%
The number as well as depth of forks witnessed by the observer significantly
varies as a function of his or her relative position with respect to the miners
in the network.
%
The need for an instability measure that accounts for the relative position of
an observer fundamentally changes the design and operation of the blockchains.


